Reverse Engineering x86 Processor Microcode

Microcode is an abstraction layer on top of the physical components of a CPU and present in most general-purpose CPUs today. In addition to facilitate complex and vast instruction sets, it also provides an update mechanism that allows CPUs to be patched in-place without requiring any special hardware. While it is well-known that CPUs are regularly updated with this mechanism, very little is known about its inner workings given that microcode and the update mechanism are proprietary and have not been throughly analyzed yet. In this paper, we reverse engineer the microcode semantics and inner workings of its update mechanism of conventional COTS CPUs on the example of AMD's K8 and K10 microarchitectures. Furthermore, we demonstrate how to develop custom microcode updates. We describe the microcode semantics and additionally present a set of microprograms that demonstrate the possibilities offered by this technology. To this end, our microprograms range from CPU-assisted instrumentation to microcoded Trojans that can even be reached from within a web browser and enable remote code execution and cryptographic implementation attacks.

==> figures/ucode_overview.tex <==
% !TEX root = ../ucode.tex

\begin{tikzpicture}
	\draw [help lines] (0,0) grid (8,7);

	\tikzstyle{block} = [draw,rectangle,black,fill=white,minimum width=8.5em,
	drop shadow={shadow xshift=1pt,shadow yshift=-1pt,fading angle=-45}]

	\tikzstyle{datapathblock} = [draw,rectangle,black,fill=white,minimum width=2.75em, minimum height=2.5em,
	drop shadow={shadow xshift=1pt,shadow yshift=-1pt,fading angle=-45}]


	\draw [rounded corners, fill=black!10, drop shadow={shadow xshift=1pt,shadow yshift=-1pt,fading angle=-45}] (0.15,2.6) rectangle (7.85,6.5);
	%\node at (1.25, 6.25) {Control Path};
	
 
	\node [block,rotate=90] (fetch) at (0.75, 4.5) {Instruction Fetch};

	\node [block,rotate=90] (ir) at (1.75, 4.5) {Instruction Register};

	\node [block,rotate=90, minimum width=7em, align=center] (start) at (3,4.5) {
		Start Addr.\\
		Generation 
	};

	\node [block,rotate=90, minimum width=7em, align=center] (sequencer) at (4.5,4.5) {
		Sequencer\\ 
		\ \\
		\
	};

	\node [block, rotate=90, minimum width=4em, text height=0.5em] (micropc) at (4.75,4.5) {\small{$\mu$PC}};

	\node [block,align=center,minimum width=5em, minimum height=7em] (rom) at (6.5, 4.5) {
		Microcode\\
		ROM\\
		\ \\
		\ \\
	};

	\foreach \y in {0.75, 1.75} {
		\node [datapathblock] (alu) at (6,\y) {ALU};
		\node [datapathblock] (ld) at (4.5,\y) {LD};
	} 
	\node [datapathblock] (st) at (3, 1.75) {ST};
	\node [datapathblock] (addr) at (3, 0.75) {ADR};

	\draw[->] (fetch) -- (ir);
	\draw[->] (ir) -- (start);
	\draw[->] (start) -- (sequencer);
	\draw[->] (sequencer) -- (rom);


\end{tikzpicture}
